TensorGPT: Efficient Compression of Large Language Models based on Tensor-Train Decomposition

High-dimensional token embeddings underpin Large Language Models (LLMs), as they can capture subtle semantic information and significantly enhance the modelling of complex language patterns. However, this high dimensionality also introduces considerable model parameters and prohibitively high model storage and memory requirements, which is particularly unaffordable for low-end devices. Targeting no extra training data and insufficient computation cases, we propose a training-free model compression approach based on the Tensor-Train Decomposition (TTD), whereby each pre-trained token embedding is converted into a lower-dimensional Matrix Product State (MPS). We then comprehensively investigate the low-rank structures extracted by this approach, in terms of the compression ratio, the language task performance, and latency on a typical low-end device (i.e. Raspberry Pi). Taking GPT family models (i.e. GPT-2 and CerebrasGPT) as case studies, our approach theoretically results in $46.89\%$ fewer parameters of the entire model, with a compression ratio $39.38\times$ - $65.64\times$ for the embedding layers. With different hyperparameter choices, the model compressed with our approach can achieve a comparable language task performance to the original model with around $2.0\times$ embedding layer compression. This empirically proves the existence of low-rank structure in GPT family models, and demonstrates that about half of the parameters in the embedding layers are redundant.

==> offcial_instructions.tex <==

\section{Submission of conference papers to ICLR 2025}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2025 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2025_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2025_conference.sty+ and \verb+iclr2025_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2025_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 10 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> sections/findings.tex <==
\section{The Low-rank Structure extracted by TensorGPT}

\begin{figure}[t]
\centering
\begin{subfigure}{0.5\textwidth}
    \includegraphics[width=\textwidth]{figures/heatmap-mae.pdf}
    \caption{Embedding weights ${\bf W}_{\texttt{emb}}$ and MAE of \cref{ttcp_alg:ttsvd}.}
    \label{fig:wte}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/centroid.pdf}
    \caption{Mass and geometric centre of tensors.}
    \label{fig:statics}
\end{subfigure}       
\caption{(a) The token embedding weights distribution across 150 tokens. The darker the pixels are, the higher the values they represent are. (b) The mass centre and the geometric centre of tensor. The tensor size of tensor $\mathcal{A}$ $\mathcal{B}$ are similar. However, their absolute distance between their mass centres ($C_{\mathcal{A}}$ and $C_{\mathcal{B}}$) and geometric centres ($O_{\mathcal{A}}$ and $O_{\mathcal{B}}$) are very different on their $3$rd mode, that is $\texttt{dist}(\mathcal{A},3)<\texttt{dist}(\mathcal{B},3)$, where $\texttt{dist}(\cdot)$ is defined in \cref{eq:abs}. }
\vspace{-10px}
\end{figure}

%In this section, we refer to the compression setting with compression ratio $0.5\times$ - $2.0\times$ and comparable language modelling performance as ``sound compression''. Based on the experimental results, we show what contributes to this sound compression and how to achieve sound compression. 

Now look back at the question we ask in \cref{sec:intro}: {\it What lower-rank structures can be extracted from the pre-trained model embedding layers?} In this section, with our proposed TensorGPT and the experimental results in \cref{sec:exp}, we will answer this question from two perspectives: 1) what information is compressed into a lower-rank structure, and 2) what features of the low-rank structure we can utilize to extract the lower-rank structure more efficiently? 

\subsection{What information is compressed?}
From \cref{sec:exp-res} we know that whatever the tensor size, there are almost some TT ranks that can result in $0.5\times$ - $2.0\times$ sound compression. This phenomenon implies that there is indeed at least one low-rank structure, whose size is around half of the original, and the rest can be compressed. To indicate possible clues of this low-rank structure, in \cref{fig:wte}, we plot the Absolute Error (AE) of the reconstructed embedding layer of maximum compression ($39.42\times$, the middle grey row) and sound compression ($0.60\times$, the lower grey row) of DistilGPT2. In the upper green row, which refers to the weights of these 150 different tokens, we find that some dimensions have similar values (indicated by light or dark vertical lines). In the middle maximum compression row, these lines are not accurately compressed, since at the same positions the colour is darker than the rest. However, in the lower sound compression row, the overall colour is darker, which means the overall reconstruction is not as accurate as the middle maximum row. The lighter lines indicate the reconstruction of these lines is more accurate. Overall, the difference of the lines reconstruction implies that in sound compression, the compressed information might be the less common pattern of the tokens, which might be the noises in the embeddings.      

% We then compressed these 150 token embeddings individually with \cref{ttcp_alg:ttsvd}, and got the Absolute Error (AE) when the compression ratio is the maximum and the compressed model has improved task performance 

\subsection{How to find the low-rank structure more efficiently?}

During the compression in \cref{ttcp_alg:ttsvd}, we have the following two kinds of hyperparameters:
\begin{enumerate}
    \item {\bf Tensor Size $\{I_1, I_2, \ldots, I_N\}$}, used for the construction of a high-dimensional tensor with the individual embedding vector;
    \item {\bf TT Ranks $\{r_0, r_1,\ldots, r_N\}$}, used is for Tensor-Train Decomposition, breaking the high-dimensional tensor into smaller tensor cores. 
\end{enumerate}

As mentioned in \cref{sec:exp-res}, almost all tensor sizes we tested have certain TT rank options that can result in around $0.5\times$ - $2.0\times$ compression ratio and language modelling perplexity less than $100.0$. However, as the combinations of the tensor sizes and the corresponding TT ranks can explode exponentially, it is impossible to test all the possible hyperparameters to achieve such a sound compression. However, there still a clue to efficiently find the hyperparameters.     

For example, in \cref{fig:statics}, the tensor sizes of two different $3$-order tensors $\mathcalbf{A}$ and $\mathcalbf{B}$ are similar, while their TT ranks for a sound compression might be different because of their different parameter distribution. In \cref{line:svd} of \cref{ttcp_alg:ttsvd}, each order is processed via truncated SVD, which means for each order the values of ``pixels'' are processed as an entity. 
Herein we can describe the distribution of a tensor with a physical term {\it mass centre} - a unique point in the tensor that represent the mean location of tensor value distribution. 

\begin{definition}[Mass Centre of Tensor]\label{def:mass} The centre of mass of a $N$-order tensor $\mathcalbf{X} \in \mathbb{R}^{I_1\times I_2 \times \cdots \times I_N}$ has the coordinate $(c_1,c_2,\ldots, c_N)$, where the $c_k (k=1,2,\ldots, N)$ can be obtained from 
\begin{equation}
    c_k = \frac{\sum^{I_k}_{t=1} \Bigl(  \sum^{I_1}_{i=1} \sum^{I_2}_{j=1}\cdots \sum^{I_N}_{k=1}    t \mathcalbf{X}[k_1,k_2,\ldots,k_N]\Bigl)}{\sum^{I_1}_{k_1=1} \sum^{I_2}_{k_2=1}\cdots \sum^{I_N}_{k_N=1}   \mathcalbf{X}[k_1,k_2,\ldots,k_N]}.
\end{equation}
\end{definition}



We can also have the definition of the geometric center  of a tensor, and the normalized absolute difference between the mass centre and the geometric centre on each order:
\begin{definition}[Geometric Center of Tensor]\label{def:centroid} The geometric centre of a $N$-order tensor $\mathcalbf{X} \in \mathbb{R}^{I_1\times I_2 \times \cdots \times I_N}$ has the coordinate $(o_1,o_2,\ldots, o_N)$, where the $o_k = \frac{1}{2}I_k(k=1,2,\ldots, N)$.
\end{definition}
\begin{definition}[Absolute Difference of Tensor]\label{eq:abs} In a $N$-order tensor $\mathcalbf{X}\in \mathbb{R}^{I_1\times I_2 \times \cdots \times I_N}$, the normalized absolute difference $\texttt{dist}(\mathcalbf{X}, k)$ for the $k$th mode of tensor $\mathcalbf{X}$ is defined as 
\begin{equation}
    \texttt{dist}(\mathcalbf{X}, k) = {|c_k - o_k|},
\end{equation}
where $c_k$ and $o_k$ are the coordinates of the mass centre and geometric centre of the $k$th mode. Then the overall distance between the geometric centre and mass centre of tensor $\mathcal{X}$ is
\begin{equation}
    \sigma(\mathcal{X})  =\sum^{\text{dim}(\mathcal{X})}_{k=1} \texttt{dist} (\mathcal{X},k)
\end{equation}

\end{definition}

For a $N$-order tensor $\mathcal{X}$, intuitively there should be certain monotonicity between absolute difference and the expressity of tensor $\mathcal{X}$. For example, the smaller absolute difference is, the geometric centre is closer to the mass centre so that the geometric centre can better approximate the mass centre, which indicates the values in $\mathcal{X}$ follows a quasi-uniform distribution. Denote $h_t$ as a hyperparameter set, $h_t = (\{I_t\},\{r_t\})$, where $\{I_t\}$ is the tensor size and $\{r_t\}$ is the TT ranks of tensor $\mathcal{X}$, respectively.

% Also, for the $k$ absolute differences of the same tensor, the order of these differences can guide the choice of TT ranks. For example, if $\texttt{dist}(\mathcalbf{X}, k_1)>\texttt{dist}(\mathcalbf{X}, k_2)$, the chosen TT ranks are easier to satisfy $r_{k_1}>r_{k_2}$, where $k_1$ and $k_2$ are two different modes.  

We investigate the compression with perplexity no more than $100.0$ and compression ratio more than $0.5\times$. As an example, in \cref{tab:trick} we listed normalized absolute differences, optimal TT ranks and its compression results, of part of $3$-order compression cases of DistilGPT2. The first two tensor sizes $(3, 8, 32)$ and $(4, 48, 4)$ with smaller normalized absolute differences are easier to find TT ranks for the above-mentioned sound compression. However, the last four, whose normalized absolute differences are larger, are unable to find a sound compression of $0.5\times$ and above compression ratio and less than $100.0$ complexity. Their possible TT ranks near this point are already listed in \cref{tab:trick}, and s slight change in the TT rank can result in unsatisfying perplexity (higher than $100.0$) or compression ratio (less than $0.5\times$).

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]\footnotesize
% \centering
% \begin{tabular}{c|c|l|l|l}
% \toprule
% $\{I_k\}$ &  $\frac{1}{N}{\sum^{N}_{k=1}\texttt{dist}(\mathcal{X},k)}$       & Optimal $\{r_k\}$          & $\eta_{\texttt{emb}}$ & $\texttt{PPL}$ \\ \midrule
% $(3, 8, 32)$ & 0.081 & $[1,3,8,1]$ &  $0.68 \times$ & 90.44 \\ \hline
% $(4, 48, 4)$ & 0.087 & $[1,3,3,1]$ &  $0.68 \times$ & 99.32 \\ \midrule
% $(6, 2, 64)$ & 0.114 & $[1,6,6,1]$ &  $0.56 \times$ & 102.30 \\ \hline
% \multirow{2}{*}{$(4, 2, 96)$} & \multirow{2}{*}{0.127} & $[1,4,5,1]$ &  $0.43 \times$ & 88.31 \\\cline{3-5}
%   & & $[1,4,4,1]$ & $0.78\times$ & 102.09 \\ \hline
% \multirow{2}{*}{$(4, 96, 2)$} & \multirow{2}{*}{0.127} & $[1,2,2,1]$ &  $0.94 \times$ & 168.40 \\\cline{3-5}
%   & & $[1,3,2,1]$ & $0.30\times$ & 85.18 \\ \hline
%  \multirow{2}{*}{$(2, 2, 192)$} & \multirow{2}{*}{0.167} & $[1,2,2,1]$ &  $0.94 \times$ & 89.40 \\\cline{3-5}
%   & & $[1,2,3,1]$ & $0.30\times$ & 84.40 \\ 
%  \bottomrule
% \end{tabular}
% \caption{Compression cases of DistilGPT2 with tensor order $N=3$.}\label{tab:trick}
% \vspace{-20px}
% \end{table}


% the tensor sizes of $\mathcalbf{A}$ and $\mathcalbf{B}$ are similar, yet their common patterns across different token embeddings dispersion (mainly in the dimension parallel with the x-axis) are different. The coordinates of the top five most similar pixels across different tokens (highlighted with orange and green squares) $\mathcalbf{B}$ are more separated in the x direction than $\mathcalbf{A}$. This gives us a clue that to find a tensor size of abundant TT ranks for sound compression, we can try the tensor sizes with more clustered coordinates of common pixels. 


% Some tensor sizes are easier to get comparable language task performance with $0.5\times$ - $2.0\times$ compression ratio, which means these tensor shapes have more TT rank choices to achieve such a kind of compression (See \x{Appendix}). 
% To quantify the properties of such a kind of tensor sizes, we set an objective function $\gamma = \frac{\Delta \ln \texttt{PPL}}{\eta_{\texttt{emb}}}$, and try to use $\gamma$ to find these tensor sizes.  
% Generally, the smaller $\gamma$ is, the better the compression is. $\gamma$ still tends to be more sensitive to perplexity, since in the logarithmic perplexity the number of the summands are more than that of the compression ratio. Thus we can set a empirical value range $[\gamma_1, \gamma_2]$ to select the reasonable $\gamma$. 

% and define a coefficient $\gamma = \frac{\Delta \ln \texttt{PPL}}{\eta_{\texttt{emb}}}$ as the objective function to find these tensor sizes. However, 











==> sections/others/table.tex <==
\begin{table}[]\small
\caption{Parameters, number of floating-point operations (flops) of the compressed and uncompressed sub-billion models, latency on Raspberry Pi CPU. ``original'' means uncompressed model, $\texttt{PPL} \leq 100.0$ means the compressed model with negligible accuracy drop, and the notation $\varphi_{\text{max}}$ refers to the compressed model with maximum compression ratio. $l_{\text{text}}$ is the number of the tokens in the input text. (s/text, $l_{\text{text}}=50$)}\label{tab:exp-profile}
\centering
\begin{tabular}{l?lll?lll?lll}
\toprule
\multicolumn{1}{c?}{\multirow{2}{*}{\textbf{GPT Series}}} & \multicolumn{3}{c?}{\textbf{\# Params} (M)}                                          & \multicolumn{3}{c?}{\textbf{flops} ($l_{\text{text}}=100$)}    &  \multicolumn{3}{c}{\textbf{Raspberry Pi latency} }                      \\ \cline{2-10} 
\multicolumn{1}{c?}{}                                & \multicolumn{1}{l|}{original} & \multicolumn{1}{l|}{$\texttt{PPL}$} & $\varphi_{\text{max}}$ & \multicolumn{1}{l|}{original(G)} & \multicolumn{1}{l|}{$\texttt{PPL}$} & $\varphi_{\text{max}}$ & \multicolumn{1}{l|}{original} & \multicolumn{1}{l|}{$\texttt{PPL}$} & $\varphi_{\text{max}}$ \\ \midrule
 \multirow{4}{*}{GPT2} & \multicolumn{1}{l|}{81.9}         & \multicolumn{1}{l|}{67.06 }                  &    43.45      & \multicolumn{1}{l|}{20.25 G}         & \multicolumn{1}{l|}{$+$ 1.65 M}                  &    $+$ 0.13 M   & \multicolumn{1}{l|}{$0.19_{\pm 0.02}$}         & \multicolumn{1}{l|}{${0.36}_{\pm 0.19}$}                  &  $0.19_{\pm 0.03}$   \\ \cline{2-10}
 & \multicolumn{1}{l|}{124.44}         & \multicolumn{1}{l|}{106.36 }                  &   85.99       & \multicolumn{1}{l|}{40.49 G}         & \multicolumn{1}{l|}{$+$ 1.88 M}                  &   $+$ 0.13 M & \multicolumn{1}{l|}{$0.50_{\pm 0.19}$}         & \multicolumn{1}{l|}{${0.50}_{\pm 0.16}$}                  &  $0.71_{\pm 0.38}$ \\ \cline{2-10}
& \multicolumn{1}{l|}{354.82}         & \multicolumn{1}{l|}{326.45 }                  &  303.88         & \multicolumn{1}{l|}{142.25 G}         & \multicolumn{1}{l|}{$+$ 3.11 M}                  &     $+$ 0.20 M  & \multicolumn{1}{l|}{$1.23_{\pm 0.12}$}         & \multicolumn{1}{l|}{$1.26_{\pm 0.22}$ }                  &  $1.55_{\pm 0.36}$  \\ \cline{2-10}
 & \multicolumn{1}{l|}{774.03}         & \multicolumn{1}{l|}{734.28}                  &   710.83      & \multicolumn{1}{l|}{330.98 G}         & \multicolumn{1}{l|}{$+$ 2.30 M}                  &          $+$ 0.25 M 
 & \multicolumn{1}{l|}{$3.01_{\pm 0.47}$}         & \multicolumn{1}{l|}{$3.01_{\pm 0.29}$}                  &   $3.52_{\pm 0.44}$        
    \\ \midrule
 \multirow{3}{*}{CerebrasGPT} & \multicolumn{1}{l|}{111.05}         & \multicolumn{1}{l|}{101.78}                  &    71.87     & \multicolumn{1}{l|}{14.47 G}         & \multicolumn{1}{l|}{$+$ 0.38 M}     &$+$ 0.13 M   & \multicolumn{1}{l|}{$0.47_{\pm 0.21}$}  & \multicolumn{1}{l|}{$0.48_{\pm 0.23}$}                  & $0.72_{\pm 0.42}$              \\ \cline{2-10}
& \multicolumn{1}{l|}{255.98}         & \multicolumn{1}{l|}{226.69}                  &    200.59     & \multicolumn{1}{l|}{40.4 G}         & \multicolumn{1}{l|}{$+$ 1.63 M }                  &   $+$ 0.12 M  & \multicolumn{1}{l|}{$0.71_{\pm 0.02}$}         & \multicolumn{1}{l|}{$1.01_{\pm 0.29}$}   & $0.95_{\pm 0.27}$ \\ \cline{2-10}
 & \multicolumn{1}{l|}{590.31}         & \multicolumn{1}{l|}{543.45}                  &    511.07     & \multicolumn{1}{l|}{103.06 G}         & \multicolumn{1}{l|}{$+$ 2.30 M}                  &     $+$ 0.26 M & \multicolumn{1}{l|}{$1.81_{\pm 0.25}$}         & \multicolumn{1}{l|}{$1.89_{\pm 0.28}$}   &  $1.91_{\pm 0.24}$
         \\ \bottomrule


         
% & \multicolumn{3}{c?}{\textbf{Server latency} (ms/text)} & \multicolumn{3}{c}{\textbf{Raspberry Pi latency} (s/text, $l_{\text{text}}=50$)}                                             \\ \cline{2-7} 
%          & \multicolumn{1}{l|}{original} & \multicolumn{1}{l|}{$\texttt{PPL} \leq 100.0 $} & $\varphi_{\text{max}}$ & \multicolumn{1}{l|}{original} & \multicolumn{1}{l|}{$\texttt{PPL} \leq 100.0 $} & $\varphi_{\text{max}}$  \\ \midrule
         
%           \multirow{4}{*}{GPT2}  &   \multicolumn{1}{l|}{35.496}         & \multicolumn{1}{l|}{$+$ 30.202}                  &  $+$ 52.200  & \multicolumn{1}{l|}{$0.19_{\pm 0.02}$}         & \multicolumn{1}{l|}{${0.36}_{\pm 0.19}$}                  &  $0.19_{\pm 0.03}$    \\ \cline{2-7}
          
%           &        \multicolumn{1}{l|}{66.719}         & \multicolumn{1}{l|}{$+$ 27.010}                  &  $+$ 51.007   & \multicolumn{1}{l|}{$0.50_{\pm 0.19}$}         & \multicolumn{1}{l|}{${0.50}_{\pm 0.16}$}                  &  $0.71_{\pm 0.38}$  \\ \cline{2-7}
          
%           &  \multicolumn{1}{l|}{200.715}         & \multicolumn{1}{l|}{$+$ 4.498}                  &  $+$ 11.815    & \multicolumn{1}{l|}{$1.23_{\pm 0.12}$}         & \multicolumn{1}{l|}{$1.26_{\pm 0.22}$ }                  &  $1.55_{\pm 0.36}$  \\ \cline{2-7}
          
%           & \multicolumn{1}{l|}{406.457}         & \multicolumn{1}{l|}{$+$ 4.278}                  &   $+$ 8.093   & \multicolumn{1}{l|}{$3.01_{\pm 0.47}$}         & \multicolumn{1}{l|}{$3.01_{\pm 0.29}$}                  &   $3.52_{\pm 0.44}$
%      \\ \midrule

     
%  \multirow{3}{*}{CerebrasGPT}  &  \multicolumn{1}{l|}{4.429} & \multicolumn{1}{l|}{}   &   & \multicolumn{1}{l|}{$0.47_{\pm 0.21}$}  & \multicolumn{1}{l|}{$0.48_{\pm 0.23}$}                  & $0.72_{\pm 0.42}$ \\ \cline{2-7}
%   & \multicolumn{1}{l|}{9.187 }         & \multicolumn{1}{l|}{}  &      & \multicolumn{1}{l|}{$0.71_{\pm 0.02}$}         & \multicolumn{1}{l|}{$1.01_{\pm 0.29}$}   & $0.95_{\pm 0.27}$  \\ \cline{2-7}
%   & \multicolumn{1}{l|}{19.817 }         & \multicolumn{1}{l|}{}  &       & \multicolumn{1}{l|}{$1.81_{\pm 0.25}$}         & \multicolumn{1}{l|}{$1.89_{\pm 0.28}$}   &  $1.91_{\pm 0.24}$
%      \\ \bottomrule
\end{tabular}
\end{table}
